Advancing Mental Health Pre-Screening: A New Custom GPT for Psychological Distress Assessment

This study introduces 'Psycho Analyst', a custom GPT model based on OpenAI's GPT-4, optimized for pre-screening mental health disorders. Enhanced with DSM-5, PHQ-8, detailed data descriptions, and extensive training data, the model adeptly decodes nuanced linguistic indicators of mental health disorders. It utilizes a dual-task framework that includes binary classification and a three-stage PHQ-8 score computation involving initial assessment, detailed breakdown, and independent assessment, showcasing refined analytic capabilities. Validation with the DAIC-WOZ dataset reveals F1 and Macro-F1 scores of 0.929 and 0.949, respectively, along with the lowest MAE and RMSE of 2.89 and 3.69 in PHQ-8 scoring. These results highlight the model's precision and transformative potential in enhancing public mental health support, improving accessibility, cost-effectiveness, and serving as a second opinion for professionals.

==> mae_table.tex <==
\begin{table}[htbp]
\centering
\caption{Results}
\small
\begin{tabular}{l|c|ccc}
\toprule
Testing Stage & Background Knowledge & MAE & RMSE & R-squared \\
\midrule
\multirow{6}{*}{Stage 1} & All & 2.89 & 3.69 & 0.67 \\
 & NoBG & 4.42 & 5.59 & 0.24 \\
 & PHQ8 & 3.28 & 4.39 & 0.53 \\
 & DSM5 & 3.98 & 5.22 & 0.33 \\
 & D5P8 & 3.04 & 4.16 & 0.58 \\
 & 4o & 4.04 & 5.4 & 0.29 \\
\multirow{6}{*}{Stage 2} & All & 2.96 & 3.81 & 0.64 \\
 & NoBG & 3.53 & 5 & 0.39 \\
 & PHQ8 & 3.32 & 4.49 & 0.51 \\
 & DSM5 & 3 & 4.19 & 0.57 \\
 & D5P8 & 2.91 & 3.98 & 0.61 \\
 & 4o & 3.45 & 4.78 & 0.44 \\
\multirow{6}{*}{Stage 3} & All & 1.53 & 2.26 & 0.88 \\
 & NoBG & 1.57 & 2.72 & 0.82 \\
 & PHQ8 & 1.68 & 2.95 & 0.79 \\
 & DSM5 & 1.57 & 2.78 & 0.81 \\
 & D5P8 & 1.64 & 2.59 & 0.84 \\
 & 4o & 1.29 & 2.44 & 0.85 \\
\bottomrule
\end{tabular}
\end{table}

==> table7.tex <==
\begin{table*}[t]
\caption{Performance comparison of Psycho Analyst Custom GPT with previous methods on DAIC-WOZ Transcript Analysis}
\label{tab:table7}
\centering
\begin{tabular}{l|l|cc}
\hline
\textbf{ } & \textbf{Approach} & \textbf{F1} & \textbf{Macro-F1} \\ \hline
Villatoro et al. (2021) \cite{villatoro2021approximating} & Mental Lexicon Features & - & 0.83 \\ 
Solieman et al. (2021) \cite{solieman2021detection} & Text-Analysis on Nondepressed Group & 0.8 & - \\ 
Belser et al. (2023) \cite{belser2023comparison} & Long-sequence Transfomer and HAM & 0.76 & - \\ 
Milintsevich et al. (2023) \cite{milintsevich2023towards} & Multi-target Hierarchical Regression Model & - & 0.74 \\ 
Yadav et al. (2023) \cite{yadav2023novel} & Bidirectional Gated Recurrent Unit (BGRU) Network & 0.92 & - \\ 
This work & Psycho Analyst Custom GPT & \textbf{0.929} & \textbf{0.949} \\ \hline
\end{tabular}
\end{table*}

